Cross-lingual Parsing with Polyglot Training and Multi-treebank Learning: A Faroese Case Study

Cross-lingual dependency parsing involves transferring syntactic knowledge from one language to another. It is a crucial component for inducing dependency parsers in low-resource scenarios where no training data for a language exists. Using Faroese as the target language, we compare two approaches using annotation projection: first, projecting from multiple monolingual source models; second, projecting from a single polyglot model which is trained on the combination of all source languages. Furthermore, we reproduce multi-source projection (Tyers et al., 2018), in which dependency trees of multiple sources are combined. Finally, we apply multi-treebank modelling to the projected treebanks, in addition to or alternatively to polyglot modelling on the source side. We find that polyglot training on the source languages produces an overall trend of better results on the target language but the single best result for the target language is obtained by projecting from monolingual source parsing models and then training multi-treebank POS tagging and parsing models on the target side.

==> discussion.tex <==






==> method_redundant.tex <==
%%: NOW REDUNDANT MOVED TO SECT 3 16:24 Aug 19th

The process used for creating a synthetic treebank for cross-lingual dependency parsing is outlined in this section.

\subsection{Corpus Translation}
\label{sec:method:translation}

Starting from the raw text extracted from Wikipedia, the target (Faroese) sentences are translated into the four source languages, firstly by translating from Faroese to Norwegian \bokmaal{} and then using pivot translation to translate between Norwegian \bokmaal{} to the other source languages.


\subsection{Synthetic Source Treebanks}
\label{sec:method:sst}

Source translations are tokenized with UDPipe by \newcite{tyers-etal-2018-multi}.
For each source language, the POS model trained on the full training data (Section~\ref{sec:data:pos}) is used
to POS tag the tokenized translations. 
Once the text is POS tagged, we predict dependencies (arcs and labels) with the parsing models of the previous section, providing syntactic annotations for these texts.


\subsection{Word Alignments}
\label{sec:method:alignment}

Word alignments between the Faroese text and the source translations are generated using fast\textunderscore{align} \cite{dyer-etal-2013-simple}, a word alignment tool based on IBM Model 2.
Note that previous related work \cite{agic-etal-2016-multilingual} reported better results using IBM Model 1 with a more diverse language setup and that IBM Model 2 introduces a bias towards more closely related languages.
As we are working with related languages and translations and alignments are largely word for word, we expect that this will have less of an impact although IBM Model 1 should also be tried in future work.

\subsection{Annotation Projection}
\label{sec:method:projection}

The annotations are then projected from the source translations to the target language using the word alignments and \citeauthor{tyers-etal-2018-multi}'s projection tool, resulting in a lexicalized target training treebank.
In some cases, not all tokens are aligned and \newcite{tyers-etal-2018-multi} work around this by falling back to a 1:1 mapping between the target index and the source index.
There are also cases where there is a mismatch in length between the source and target sentences and some dependency structures cannot be projected to the target language.
\citeauthor{tyers-etal-2018-multi}'s projection tool excludes unsuitable projected trees containing \eg more than one root token, a token that is its own head or a token with a head outside the range of the sentence from its output.

\subsection{Multi-source Projection}
\label{sec:multi-source}

For multi-source projection, the four source-language dependency trees for a Faroese sentence are projected into a single graph, scoring edges according to the number of trees that contain them.
The resulting Faroese dependency tree is decoded using MST arc-voting based on majority vote \cite{ sagae-lavie-2006-parser, nivre-etal-2007-conll}.


\subsection{Target Language POS Tagging and Parsing Models}
Finally, plain and multi-treebank target-language POS tagging parsing models are trained on the newly created treebank(s) and are used to POS tag and parse the target test treebank.


==> results-full.tex <==
\begin{table*}[t!]
\centering
\small
%\fontsize{8}{10}\selectfont
\begin{tabular}{*{10}{l}}
\toprule
%---------- headers
\sc Source Language & \sc Model & \multicolumn{3}{c}{\sc Single} & \multicolumn{2}{c}{\sc Multi-TB} & \multicolumn{3}{c}{\sc Multi-TB + POS}  \\
%\cmidrule(lr){1-2}
\cmidrule(lr){3-5}
\cmidrule(lr){6-7}
\cmidrule(lr){8-10}
& & \sc UPOS & \sc UAS & \sc LAS & \sc UAS & \sc LAS & \sc UPOS & \sc UAS & \sc LAS \\
%---------
\multirow{2}{*}{\sc Danish}
        & Monolingual & \bf 73.02 & 69.66 & 61.24 & 70.72 & 62.39 & 71.45 & 71.8 & 63.4 \\%

        & Polyglot & 71.1 & \bf 74.32 & 65.29 &  73.88 & 65.12 & 72.48 & 73.95 & \bf 65.53 \\%
\addlinespace
\multirow{2}{*}{\sc Swedish}
        & Monolingual & 70.99 & 73.53 & 65.93 &  72.25 & 64.95 & \bf 72.57 & 73.07 & 66.15 \\%

        & Polyglot & 71.27 & 75.93 & 68.6 &  76.05 & 69.03 & 71.84 & \bf 76.37 & \bf 69.69 \\%
\addlinespace
\multirow{2}{*}{\sc Norwegian Nynorsk}
        & Monolingual & 77.04 & 77.36 & 70.27 &  78.03 & 70.93 & 77.4 & \bf 78.66 & \bf 71.51 \\%

        & Polyglot & 76.88 & 77.08 & 69.8 &  77.71 & 70.72 & \bf 77.58 & 77.97 & 71.13 \\%
\addlinespace
\multirow{2}{*}{\sc Norwegian \bokmaal{}}
        & Monolingual & \bf 74.62 & 75.09 & 67.46 &  75.53 & 67.8 & 74.39 & 75.73 & 67.94 \\%

        & Polyglot & 74.21 & \bf 77.86 & 70.51 &  77.53 & 70.43 & 74.53 & 77.4 & \bf 70.58 \\%
\addlinespace
\multirow{2}{*}{\sc Multi-source}
        & Monolingual & 71.76 & 77.33 & 68 &  77.76 & 68.65 & \bf 72.65 & 78.02 & 69.8 \\%

        & Polyglot & 71.16 & 76.95 & 68.55 &  78.35 & 69.22 & 72.04 & \bf 78.86 & \bf 70.07 \\%
\addlinespace
\multirow{2}{*}{\sc Average}
        & Monolingual & 73.49 & 74.59 & 66.58 &  74.86 & 66.94 & \bf 73.69 & 75.46 & 67.76 \\%

        & Polyglot & 72.92 & 76.43 & 68.55 &  76.70 & 68.90 & \bf 73.69 & \bf 76.91 & \bf 69.40 \\%
\addlinespace
%\cmidrule(lr){3-5}
%\cmidrule(lr){6-7}
%\cmidrule(lr){8-10}
\bottomrule
\end{tabular}
%\end{center}
\caption{\label{table:results-faroese} POS accuracy, UAS and LAS on the target Faroese test treebank. The polyglot model is tested with each of the five training treebanks (four projected from individual source languages and one using multi-source projection) as proxy treebank.}
\end{table*}
